Feasibility Study for BioLEIR

The biomedical community asked CERN to investigate the possibility to transform the Low Energy Ion Ring (LEIR) accelerator into a multidisciplinary, biomedical research facility (BioLEIR) that could provide ample, high-quality beams of a range of light ions suitable for clinically oriented fundamental research on cell cultures and for radiation instrumentation development. BioLEIR would be operated when LEIR is not providing heavy ions for the CERN physics programme. The study group was mandated to write a Feasibility Study Report, using high-level engineering estimates based on previous experience, with the aim to: - collect the requirements for such a facility from the biomedical community in close collaboration with the International Strategy Committee for CERN Medical Applications; - determine a coherent set of beam parameters, based on the requirements; - explore whether the beam requirements can be met throughout the facility, from the source to the biomedical end-stations; - perform a feasibility study of the facility, taking into consideration the overall CERN schedules and programmes; - favour simplicity and robustness of the facility design, while minimizing the cost of maintenance and operation; - establish a high-level costing of material and personnel needed for project implementation; - describe the preferred installation scenario; - perform a high-level risk analysis for the project; - identify the areas of potential difficulty, and the required R&D should the study go ahead and become a project.

==> contributors.tex <==
\begin{center}                       
% authors
\vskip 10.5em
\textbf{BioLEIR Design Study Team} \\
all study team members\\
all contributors (in one way or another)\\
to be completed\\
...
\vskip 1.5em
\end{center}


==> coverpage.tex <==
\label{module_doc}

\def\documentlabel#1{\gdef\@documentlabel{#1}}
\gdef\@documentlabel{\texttt{Preliminary draft}}
\documentlabel{CERN/ATS/... \\ (Rev. 1.2)}

\begin{titlepage}

\begin{center}\normalsize
EUROPEAN LABORATORY FOR PARTICLE PHYSICS
\end{center}
%\vskip 0.5cm

\begin{flushright}
\@documentlabel \\                   % document label
\end{flushright}
%\vskip 1cm

\begin{center}\LARGE                 % document title
\textbf{BioLEIR \\ Conceptual Design Report } \\
\end{center}
\vskip 1.5em

\begin{center}                       % authors
BioLEIR Design Study Team \\
Sharif Ghithan, Ghislain Roy, Silvia Schuh (editors)
\vskip 1.5em

{\large Abstract}
\end{center}
\begin{quotation}
The biomedical community asked CERN to investigate the possibility to transform the LEIR accelerator into a world-class radiobiological research facility (BioLEIR) that could provide ample, high-quality beams of a range of light ions suitable for multidisciplinary clinically oriented research on cell structures and for radiation instrumentation development. BiolEIR would be operated when LEIR is not used to provide heavy ions for the CERN physics programme. The study group was mandated to write a Conceptual Design Report with minimal resources, using high-level engineering estimates based on previous experience, with the aim to:
\begin{itemize}
	\item establish the requirements for such a facility from the biomedical community in close collaboration with the International Strategy Committee of CERN Medical Applications; 
    \item determine a coherent set of beam parameters, based on the requirements;
    \item explore whether the beam requirements can be met throughout the facility, from the source to the biomedical end-stations;
    \item perform a conceptual study of the facility, taking into consideration the overall CERN schedules and programmes;
	\item favor simplicity and robustness of the facility design, while minimizing the cost of maintenance and operation;
    \item establish a high-level costing of material and people-power needed for project implementation;
    \item arrive at possible installation scenarios;
    \item perform a high-level risk analysis for the project.
    \item identify the areas of potential difficulty, and the required R\&D should the study go ahead and become a project.
\end{itemize}
The study found no show-stopper for the BioLEIR facility that could be established at LEIR to be operational just after LS2 if a decision is taken in early 2017. 
\end{quotation}
\vfill
\vskip 1.em
\begin{center}
Geneva, Switzerland \\
\today
\end{center}

\end{titlepage}

